Masked Autoencoding for Scalable and Generalizable Decision Making

We are interested in learning scalable agents for reinforcement learning that can learn from large-scale, diverse sequential data similar to current large vision and language models. To this end, this paper presents masked decision prediction (MaskDP), a simple and scalable self-supervised pretraining method for reinforcement learning (RL) and behavioral cloning (BC). In our MaskDP approach, we employ a masked autoencoder (MAE) to state-action trajectories, wherein we randomly mask state and action tokens and reconstruct the missing data. By doing so, the model is required to infer masked-out states and actions and extract information about dynamics. We find that masking different proportions of the input sequence significantly helps with learning a better model that generalizes well to multiple downstream tasks. In our empirical study, we find that a MaskDP model gains the capability of zero-shot transfer to new BC tasks, such as single and multiple goal reaching, and it can zero-shot infer skills from a few example transitions. In addition, MaskDP transfers well to offline RL and shows promising scaling behavior w.r.t. to model size. It is amenable to data-efficient finetuning, achieving competitive results with prior methods based on autoregressive pretraining.

==> tables/multi_goal.tex <==

\begin{table}[]
\begin{tabular}{|c|cc|ccc|cc|c|}
\hline
Domain          & \multicolumn{2}{c|}{Quadruped} & \multicolumn{3}{c|}{Walker} & \multicolumn{2}{c|}{Cheetah} & Average \\ \hline
Task            & run            & walk          & run      & walk    & stand  & run       & run backward     &         \\ \hline
BC              & 17.913         & 21.905        & 7.587    & 5.369   & 3.639  & 1.451     & 1.402            & 8.46      \\ \hline
Goal-GPT        & 18.017         & 21.703        & 7.972    & 5.806   & 3.646  & 2.469     & 2.687            & 8.90       \\ \hline
Ours (parallel) & 13.952         & 15.35         & 10.469   & 6.614   & 3.294  & 1.857     & 1.344            & 7.55       \\ \hline
Ours (replan)   & 12.899         & 14.775        & 5.475    & 4.767   & 2.56   & 1.879     & 1.245            & 6.23       \\ \hline
\end{tabular}
\end{table}

==> tables/single_goal.tex <==
\begin{table}[]
\begin{tabular}{|c|cc|ccc|cc|c|}
\hline
Domain          & \multicolumn{2}{c|}{Quadruped} & \multicolumn{3}{c|}{Walker} & \multicolumn{2}{c|}{Cheetah} & Average \\ \hline
Task            & run            & walk          & run     & walk    & stand   & run       & run backward     &         \\ \hline
Goal-BC              & 17.9173        & 21.7919       & 7.1277  & 5.0853  & 3.4242  & 1.158     & 1.1789           & 8.24    \\ \hline
Goal-GPT        & 17.511         & 22.185        & 7.907   & 5.435   & 3.654   & 2.465     & 2.694            & 8.84    \\ \hline
Ours (parallel) & 14.116         & 15.563        & 8.969   & 5.941   & 3.021   & 1.799     & 1.535            & 7.28    \\ \hline
Ours (replan)   & 13.428         & 15.151        & 6.595   & 3.011   & 2.322   & 1.243     & 0.8304           & 6.08    \\ \hline
\end{tabular}
\end{table}
